Dual Cross-Attention for Medical Image Segmentation

We propose Dual Cross-Attention (DCA), a simple yet effective attention module that is able to enhance skip-connections in U-Net-based architectures for medical image segmentation. DCA addresses the semantic gap between encoder and decoder features by sequentially capturing channel and spatial dependencies across multi-scale encoder features. First, the Channel Cross-Attention (CCA) extracts global channel-wise dependencies by utilizing cross-attention across channel tokens of multi-scale encoder features. Then, the Spatial Cross-Attention (SCA) module performs cross-attention to capture spatial dependencies across spatial tokens. Finally, these fine-grained encoder features are up-sampled and connected to their corresponding decoder parts to form the skip-connection scheme. Our proposed DCA module can be integrated into any encoder-decoder architecture with skip-connections such as U-Net and its variants. We test our DCA module by integrating it into six U-Net-based architectures such as U-Net, V-Net, R2Unet, ResUnet++, DoubleUnet and MultiResUnet. Our DCA module shows Dice Score improvements up to 2.05% on GlaS, 2.74% on MoNuSeg, 1.37% on CVC-ClinicDB, 1.12% on Kvasir-Seg and 1.44% on Synapse datasets. Our codes are available at: https://github.com/gorkemcanates/Dual-Cross-Attention

==> 3_RelatedWork.tex <==
\section{Related Work}
\label{sec:relatedwork}
\subsection{U-Net based Methods for Medical Image Segmentation}

U-Net \cite{ronneberger2015u} has significantly outperformed previous FCNs by introducing skip-connections which can help the decoder recover the context lost occurred in the earlier stages of the network. Motivated by the success of U-Net, several extensions have been proposed. Milletari \textit{et al.} \cite{milletari2016v} introduced V-Net for volumetric medical image segmentation using 3D convolutions and skip-connections. Zhou \textit{et al.} \cite{zhou2018unet++} proposed U-Net++, where plain skip-connections are replaced with a series of nested, dense skip pathways for further enhancing low-level encoder features before fusing them with the decoder features. Alom \textit{et al.} \cite{alom2018recurrent} proposed R2U-Net based on residual \cite{he2016deep} and recurrent \cite{liang2015recurrent} convolutions to improve the feature representation capability in U-Net. Schlemper \textit{et al.} \cite{schlemper2019attention} Attention U-Net by applying attention \cite{jetley2018learn} to further extract the salient regions on encoder features before fusing them with the decoder counterparts. Based on residual U-Net \cite{zhang2018road} and pyramid attention network \cite{li2018pyramid}, Jha \textit{et al.} \cite{jha2019resunet++} proposed ResUnet++. Their model also takes advantage of squeeze and excitation (SE) blocks \cite{hu2018squeeze} and atrous spatial pyramid pooling (ASPP) \cite{chen2017deeplab} to further improve residual U-Net. Jha \textit{et al.} \cite{jha2020doubleu} introduced DoubleU-Net, where two U-Net architectures stacked on top of each other to capture more semantic information. The first U-Net uses VGG-19 \cite{simonyan2014very} network pre-trained on ImageNet \cite{russakovsky2015imagenet} for better feature extraction. Meanwhile, the second U-Net is built from scratch to produce the final predictions. Ibtehaz \textit{et al.} \cite{ibtehaz2020multiresunet} proposed MultiResUnet to solve the semantic gap problem by incorporating residual paths between the encoder and decoder stages. These residual paths incorporate a series of convolutional layers with residual connections which help the model to recover the contextual loss that occurred in the encoder stage. MultiResUnet achieved major improvements over U-Net on different medical image segmentation datasets. Despite the notable performance of residual paths, we will show that a semantic gap still exists and even such designs over plain skip-connections can significantly be improved by our DCA mechanism.

\subsection{Transformers in Medical Image Segmentation}

Recently, transformers gained a place among FCN-based methods for medical image segmentation. TransUnet \cite{chen2021transunet} is the first study that successfully incorporates transformers into the U-Net architecture by integrating transformer layers into the encoder. TransFuse \cite{zhang2021transfuse} proposed to fuse transformers and CNNs in a parallel manner to capture both global dependency and low-level context. Cao \textit{et al.} \cite{cao2023swin} proposed Swin-Unet, the first pure transformer architecture based on swin transformer \cite{liu2021swin} for medical image segmentation. Similar to Swin-Unet, DS-TransUNet \cite{lin2022ds} was proposed to effectively combine the hierarchical swin transformer with U-Net. Moreover, several studies proposed to combine transformers with FCNs by integrating them into the encoder \cite{valanarasu2021medical, tang2022self, xu2021levit, hatamizadeh2022unetr}, decoder \cite{li2022more} or both \cite{huang2021missformer, zhou2021nnformer, naderi2022focal}.
More comprehensive analysis regarding these transformers as well as many others can be found in \cite{shamshad2022transformers, li2023transforming}. Note that our proposed method differs from such transformer-based models since our aim is to enhance skip-connections in FCNs by leveraging a cross-attention scheme at a minimal parameter increase rather than developing an end-to-end network based on transformers.



==> figs/table1.tex <==
\begin{table*}[]
\centering
\caption{Performance comparison for plain and DCA integrated models on different datasets using DSC and IoU metrics. Boldfaced results indicate better results.}
\label{table1}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{|cccccccccccc|}
\hline
\multicolumn{2}{|l}{}                                                           & \multicolumn{2}{c}{\textbf{GlaS}}                 & \multicolumn{2}{c}{\textbf{MoNuSeg}}              & \multicolumn{2}{c}{\textbf{CVC-ClinicDB}}         & \multicolumn{2}{c}{\textbf{Kvasir-Seg}}           & \multicolumn{2}{c|}{\textbf{Synapse}}              \\ \hline
\multicolumn{1}{|c|}{Model}                       & \multicolumn{1}{l|}{Params} & \multicolumn{1}{l}{DSC (\%)} & \multicolumn{1}{l}{IoU (\%)} & \multicolumn{1}{l}{DSC (\%)} & \multicolumn{1}{l}{IoU (\%)} & \multicolumn{1}{l}{DSC (\%)} & \multicolumn{1}{l}{IoU (\%)} & \multicolumn{1}{l}{DSC (\%)} & \multicolumn{1}{l}{IoU (\%)} & \multicolumn{1}{l}{DSC (\%)} & \multicolumn{1}{l|}{IoU (\%)} \\ \hline
\multicolumn{1}{|c|}{U-Net}                       & \multicolumn{1}{c|}{8.64M}  & 88.87                  & 79.98                  & 77.14                  & 62.79                  & \textbf{89.63}         & \textbf{81.43}         & 82.99                  & 71.01                  & 78.55                  & 67.37                   \\
\multicolumn{1}{|c|}{\textbf{U-Net (DCA)}}        & \multicolumn{1}{c|}{8.75M}  & \textbf{89.66}         & \textbf{81.29}         & \textbf{78.13}         & \textbf{64.11}         & 89.53                  & 81.28                  & \textbf{84.03}         & \textbf{72.53}         & \textbf{78.98}         & \textbf{67.97}          \\
\multicolumn{1}{|c|}{ResUnet++}                   & \multicolumn{1}{c|}{13.1M}  & 85.43                  & 74.62                  & 75.68                  & 60.87                  & 89.46                  & 81.14                  & \textbf{82.26}         & \textbf{69.93}         & 75.91                  & 64.61                   \\
\multicolumn{1}{|c|}{\textbf{ResUnet++ (DCA)}}    & \multicolumn{1}{c|}{13.1M}  & \textbf{87.35}         & \textbf{77.56}         & \textbf{77.40}         & \textbf{63.13}         & \textbf{90.19}         & \textbf{82.32}         & 82.07                  & 69.74                  & \textbf{77.35}         & \textbf{66.43}          \\
\multicolumn{1}{|c|}{MultiResUnet}                & \multicolumn{1}{c|}{7.24M}  & \textbf{88.99}         & \textbf{80.18}         & 76.99                  & 62.59                  & 89.52                  & 81.35                  & 81.34                  & 68.66                  & 78.12                  & 67.30                   \\
\multicolumn{1}{|c|}{\textbf{MultiResUnet (DCA)}} & \multicolumn{1}{c|}{7.35M}  & 88.86                  & 79.98                  & \textbf{78.52}         & \textbf{64.63}         & \textbf{89.95}         & \textbf{81.91}         & \textbf{82.32}         & \textbf{70.00}         & \textbf{79.50}         & \textbf{68.65}          \\
\multicolumn{1}{|c|}{R2Unet}                      & \multicolumn{1}{c|}{9.78M}  & 85.16                  & 74.26                  & 78.20                  & 64.20                  & 88.12                  & 78.88                  & 81.07                  & 68.28                  & 75.86                  & 63.94                   \\
\multicolumn{1}{|c|}{\textbf{R2Unet (DCA)}}       & \multicolumn{1}{c|}{9.89M}  & \textbf{87.21}         & \textbf{77.37}         & \textbf{78.52}         & \textbf{64.64}         & \textbf{88.39}         & \textbf{79.28}         & \textbf{82.19}         & \textbf{69.89}         & \textbf{75.90}         & \textbf{64.85}          \\
\multicolumn{1}{|c|}{V-Net}                       & \multicolumn{1}{c|}{35.97M} & 88.78                  & 79.85                  & 74.79                  & 59.74                  & 88.09                  & 79.02                  & 80.79                  & 68.07                  & 79.27                  & 68.58                   \\
\multicolumn{1}{|c|}{\textbf{V-Net (DCA)}}        & \multicolumn{1}{c|}{36.08M} & \textbf{89.03}         & \textbf{80.27}         & \textbf{77.53}         & \textbf{63.31}         & \textbf{89.46}         & \textbf{81.07}         & \textbf{81.92}         & \textbf{69.53}         & \textbf{79.58}         & \textbf{69.00}          \\
\multicolumn{1}{|c|}{DoubleUnet}                  & \multicolumn{1}{c|}{29.68M} & 89.07                  & 80.30                   & 77.16                  & 62.82                  & 90.20                  & 82.35                  & 84.40                  & 73.08                  & 79.76                  & 69.31                   \\
\multicolumn{1}{|c|}{\textbf{DoubleUnet (DCA)}}   & \multicolumn{1}{c|}{30.68M} & \textbf{89.90}         & \textbf{81.68}         & \textbf{79.50}         & \textbf{65.97}         & \textbf{90.86}         & \textbf{83.47}         & \textbf{85.16}         & \textbf{74.34}         & \textbf{80.22}         & \textbf{69.80}          \\ \hline
\end{tabular}
\end{table*}

==> figs/table2.tex <==
\begin{table}[]
\renewcommand\arraystretch{1.2}
\scriptsize
\label{table2}
\begin{center}

\begin{tabular}{|cccccc|}
\hline
\multicolumn{2}{|l}{}                                               & \multicolumn{2}{c}{\textbf{GlaS}} & \multicolumn{2}{c|}{\textbf{MoNuSeg}} \\ \hline
\multicolumn{1}{|c|}{Model}           & \multicolumn{1}{c|}{Params} & DSC (\%)             & IoU (\%)             & DSC (\%)               & IoU (\%)               \\ \hline
\multicolumn{1}{|c|}{U-Net}           & \multicolumn{1}{c|}{8.64M}  & 88.87          & 79.98          & 77.14            & 62.79            \\
\multicolumn{1}{|c|}{U-Net (CCA)}     & \multicolumn{1}{c|}{8.74M}  & 89.07          & 80.31          & 77.78            & 63.64            \\
\multicolumn{1}{|c|}{U-Net (SCA)}     & \multicolumn{1}{c|}{8.74M}  & 89.48          & 80.96          & 77.36            & 63.07            \\
\multicolumn{1}{|c|}{U-Net (SCA-CCA)} & \multicolumn{1}{c|}{8.75M}  & 89.03          & 80.24          & 77.90             & 63.80             \\
\multicolumn{1}{|c|}{U-Net (CCA-SCA)} & \multicolumn{1}{c|}{8.75M}  & \textbf{89.66} & \textbf{81.29} & \textbf{78.13}   & \textbf{64.11}   \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of different DCA layouts}
\end{table}

==> figs/table3.tex <==
\begin{table}[]
\caption{Comparison of different fusion strategies for CCA and SCA}
\label{table3}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|cccccc|}
\hline
\multicolumn{2}{|c}{}                                                & \multicolumn{2}{c}{\textbf{GlaS}}          & \multicolumn{2}{c|}{\textbf{MoNuSeg}}      \\ \hline
\multicolumn{1}{|c|}{Model}            & \multicolumn{1}{c|}{Params} & DSC (\%)             & IoU (\%)             & DSC (\%)             & IoU (\%)             \\ \hline
\multicolumn{1}{|c|}{U-Net}            & \multicolumn{1}{c|}{8.75M}  & 88.87          & 79.98          & 77.14          & 62.79          \\
\multicolumn{1}{|c|}{U-Net (CCA+SCA)}  & \multicolumn{1}{c|}{8.75M}  & 89.09          & 80.38          & 77.30          & 63.00          \\
\multicolumn{1}{|c|}{U-Net (CCA\(\vert \vert\)SCA)} & \multicolumn{1}{c|}{8.75M}  & 89.19          & 80.52          & 78.03          & 63.97          \\
\multicolumn{1}{|c|}{U-Net (CCA-SCA)}  & \multicolumn{1}{c|}{8.75M}  & \textbf{89.66} & \textbf{81.29} & \textbf{78.13} & \textbf{64.11} \\ \hline
\end{tabular}
\end{table}

==> figs/table4.tex <==
\begin{table}[]
\caption{Comparison of average pooling and convolution for patch embedding}
\label{table4}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|cccccc|}
\hline
\multicolumn{2}{|c}{}                                                & \multicolumn{2}{c}{\textbf{GlaS}}          & \multicolumn{2}{c|}{\textbf{MoNuSeg}}      \\ \hline
\multicolumn{1}{|c|}{Model}            & \multicolumn{1}{c|}{Params} & DSC (\%)             & IoU (\%)             & DSC (\%)             & IoU (\%)             \\ \hline
\multicolumn{1}{|c|}{U-Net}            & \multicolumn{1}{c|}{8.64M}  & 88.87          & 79.98          & 77.14          & 62.79          \\
\multicolumn{1}{|c|}{U-Net (DCA-Conv)} & \multicolumn{1}{c|}{9.01M}  & 89.52          & 81.07          & 77.62          & 63.43          \\
\multicolumn{1}{|c|}{U-Net (DCA-AP)}   & \multicolumn{1}{c|}{8.75M}  & \textbf{89.66} & \textbf{81.29} & \textbf{78.13} & \textbf{64.11} \\ \hline
\end{tabular}
\end{table}
